Learning to Ignore Adversarial Attacks

Despite the strong performance of current NLP models, they can be brittle against adversarial attacks. To enable effective learning against adversarial inputs, we introduce the use of rationale models that can explicitly learn to ignore attack tokens. We find that the rationale models can successfully ignore over 90% of attack tokens. This approach leads to consistent sizable improvements ($\sim$10%) over baseline models in robustness on three datasets for both BERT and RoBERTa, and also reliably outperforms data augmentation with adversarial examples alone. In many cases, we find that our method is able to close the gap between model performance on a clean test set and an attacked test set and hence reduce the effect of adversarial attacks.

==> tables/big-table-no-squad.tex <==
% Please add the following required packages to your document preamble: 
% \usepackage{booktabs} 
% \usepackage{multirow} 
\begin{table*}[t] 
% \small
\centering 
% \begin{tabular}{@{}lllllll@{}} 
% \toprule 
% Model & Architecture & Augmentation & Multirc & M. Adv. & Fever & F. Adv. \\ \midrule 
% \multirow{5}{*}{BERT} & \multirow{2}{*}{Classification} & None & 68.6& 62.6& 88.2& 78.9\\ 
% & & \dataaug & 67.3& 61.6& \textbf{88.5}& 84.8\\ \cmidrule(l){2-7} 
% & \multirow{3}{*}{Rationale} & \humantokens & 70.0& 64.4& 88.0& 76.7\\ 
% & & \dataaugwithnatokens & 69.6& 66.2& 87.1& \textbf{87.7}\\ 
% & & \dataaugwithhuman & \textbf{70.5}& \textbf{69.4}& 87.5& 87.5\\ \midrule 
% \multirow{5}{*}{RoBERTa} & \multirow{2}{*}{Classification} & None & 82.6& 76.5& 93.5& 83.0\\ 
% & & \dataaug & 84.4& 82.9& 93.2& 92.7\\ \cmidrule(l){2-7} 
% & \multirow{3}{*}{Rationale} & \humantokens & 84.0& 74.9& 94.1& 85.7\\ 
% & & \dataaugwithnatokens & \textbf{85.2}& \textbf{85.1}& \textbf{93.4}& \textbf{93.4}\\ 
% & & \dataaugwithhuman & 85.0& 82.5& \textbf{93.4}& \textbf{93.4} \\ \bottomrule 
% \end{tabular} 
\small
\begin{tabular}{lllllll}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{1}{c}{\multirow{2}{*}{Architecture}} & \multicolumn{1}{c}{\multirow{2}{*}{Training}} & \multicolumn{2}{c}{\multirc}   & \multicolumn{2}{c}{\fever}     \\ \cline{4-7} 
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                              & \multicolumn{1}{c}{}                          & Clean         & Attacked        & Clean         & Attacked        \\ \hline
\multirow{5}{*}{\bert}                      & \multirow{3}{*}{Standard}                         & \nodataaug                                      & 68.6          & 62.6          & 88.2          & 78.9          \\
                                           &                                                   & \dataaug                       & 67.3          & 61.6          & \textbf{88.5} & 84.8          \\
                                           &                                                   & \dataaugtenx                       & 66.2          & 65.9          & 86.3 & 84.5          \\ \cline{2-7} 
                                           & \multirow{3}{*}{Rationale}                        & \humantokensintable                   & 70.0          & 64.4          & 88.0          & 76.7          \\
                                           &                                                   & \dataaugwithnatokens           & 69.6          & 66.2          & 87.1          & \textbf{87.7} \\
                                           &                                                   & \dataaugwithhuman              & \textbf{70.5} & \textbf{69.4} & 87.5          & 87.5          \\ \hline
\multirow{5}{*}{\roberta}                   & \multirow{3}{*}{Standard}                         & \nodataaug                                      & 82.6          & 76.5          & 93.5          & 83.0          \\
                                           &                                                   & \dataaug                       & 84.4          & 82.9          & 93.2          & 92.7          \\
                                           &                                                   & \dataaugtenx                       & 83.5          & 82.1          & 93.5          & 93.2          \\   \cline{2-7} 
                                           & \multirow{3}{*}{Rationale}                        & \humantokensintable                   & 84.0          & 74.9          & \textbf{94.1}          & 85.7          \\
                                           &                                                   & \dataaugwithnatokens           & \textbf{85.2} & \textbf{85.1} & 93.4 & \textbf{93.4} \\
                                           &                                                   & \dataaugwithhuman              & 85.0          & 82.5          & 93.4 & \textbf{93.4} \\ \hline
\end{tabular}

\caption{Model accuracy on clean and attacked test sets for \multirc and \fever.} 
\label{tab:accuracy_table} 
\end{table*} 


==> tables/f1_new.tex <==
\begin{table*}[]
\begin{tabular}{llllll}
\hline
Model                                                       & Augmentation                        & \begin{tabular}[c]{@{}l@{}}Attack\\ F1\end{tabular} & \begin{tabular}[c]{@{}l@{}}Attack\\ F1 Corr.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Human\\ F1\end{tabular} & \begin{tabular}[c]{@{}l@{}}Human\\ F1 Corr.\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Bert Rationale\end{tabular}    & \humantokens         & 1.2                                                 & 0.046                                                     & 34.2                                               & 0.100                                                    \\
                                                            & \dataaugwithnatokens & 96.7                                                & -0.054                                                    & 29.7                                               & 0.002                                                    \\
                                                            & \dataaugwithhuman    & 11.5                                                & 0.034                                                     & 57.7                                               & 0.086                                                    \\ \hline
\begin{tabular}[c]{@{}l@{}}RoBERTa Rationale\end{tabular} & \humantokens         & 0.7                                                 & 0.054                                                     & 40.3                                               & 0.144                                                    \\
                                                            & \dataaugwithnatokens & 87.0                                                & -0.013                                                    & 29.6                                               & -0.018                                                   \\
                                                            & \dataaugwithhuman    & 8.7                                                 & 0.051                                                     & 54.4                                               & 0.108                                                    \\ \hline
\end{tabular}
\end{table*}



==> tables/f1_ver2.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% \begin{table*}[]
% \centering
% \begin{tabular}{@{}llrrrrrr@{}}
% \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{Model}} &
%   \multicolumn{1}{c}{\multirow{2}{*}{Training}} &
%   \multicolumn{3}{l}{MultiRC} &
%   \multicolumn{3}{l}{FEVER} \\ \cmidrule(l){3-8} 
% \multicolumn{1}{c}{} &
%   \multicolumn{1}{c}{} &
%   \multicolumn{1}{l}{Human (Clean)} &
%   \multicolumn{1}{l}{Attack} &
%   \multicolumn{1}{l}{Human} &
%   \multicolumn{1}{l}{Human (Clean)} &
%   \multicolumn{1}{l}{Attack} &
%   \multicolumn{1}{l}{Human} \\ \midrule
% \multirow{3}{*}{\bert} & \humantokens         & 54.5 & 11.2 & 35.8 & 80.5 & 29.6 & 65.0 \\
%                                 & \dataaugwithnatokens & 57.8 & 97.4 & 98.6 & 75.4 & 96.1 & 97.5 \\
%                                 & \dataaugwithhuman    & 59.1 & 89.3 & 57.6 & 83.4 & 95.8 & 81.9 \\ \midrule
% \multirow{3}{*}{\roberta}      & \humantokens         & 69.6 & 5.6  & 46.6 & 83.1 & 35.3 & 50.0 \\
%                                 & \dataaugwithnatokens & 69.1 & 92.1 & 97.3 & 84.1 & 94.5 & 97.4 \\
%                                 & \dataaugwithhuman    & 65.0 & 65.9 & 57.5 & 85.8 & 95.3 & 84.9 \\ \bottomrule
% \end{tabular}
% \caption{}
% \label{tab:my-table}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% \centering
% \begin{tabular}{llrrrr}
% \hline
% \multicolumn{1}{c}{\multirow{2}{*}{Model}} &
%   \multicolumn{1}{c}{\multirow{2}{*}{Training}} &
%   \multicolumn{2}{l}{MultiRC} &
%   \multicolumn{2}{l}{FEVER} \\ \cline{3-6} 
% \multicolumn{1}{c}{} &
%   \multicolumn{1}{c}{} &
%   \multicolumn{1}{l}{Attack \%} &
%   \multicolumn{1}{l}{Non-Attack \%} &
%   \multicolumn{1}{l}{Attack \%} &
%   \multicolumn{1}{l}{Non-Attack \%} \\ \hline
% \multirow{3}{*}{Bert Rationale} & \humantokens         & 87.5 & 8.2  & 66.7 & 17.8 \\
%                                 & \dataaugwithnatokens & 1.4  & 98.4 & 0.2  & 96.7 \\
%                                 & \dataaugwithhuman    & 9.5  & 14.4 & 0.5  & 24.4 \\ \hline
% \multirow{3}{*}{Rationale}      & \humantokens         & 92.4 & 12.6 & 60.0 & 12.2 \\
%                                 & \dataaugwithnatokens & 6.0  & 96.7 & 0.9  & 95.8 \\
%                                 & \dataaugwithhuman    & 32.1 & 15.6 & 0.1  & 23.0 \\ \hline
% \end{tabular}
% \caption{}
% \label{tab:my-table}
% \end{table*}

\begin{table*}[]
\begin{tabular}{llllll}
\hline
Model                                                       & Augmentation                        & \begin{tabular}[c]{@{}l@{}}Attack\\ Recall\end{tabular} & \begin{tabular}[c]{@{}l@{}}Attack\\ Recall Corr.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Human\\ Recall\end{tabular} & \begin{tabular}[c]{@{}l@{}}Human\\ Recall Corr.\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}\bert \end{tabular}    & \humantokens         & 11.2                                                    & 0.032                                                         & 35.8                                                   & 0.104                                                        \\
                                                            & \dataaugwithnatokens & 97.4                                                    & -0.055                                                        & 98.6                                                   & -0.011                                                       \\
                                                            & \dataaugwithhuman    & 89.3                                                    & -0.053                                                        & 57.6                                                   & 0.092                                                        \\ \hline
\begin{tabular}[c]{@{}l@{}}\roberta \end{tabular} & \humantokens         & 5.6                                                     & 0.043                                                         & 46.6                                                   & 0.148                                                        \\
                                                            & \dataaugwithnatokens & 92.1                                                    & -0.029                                                        & 97.3                                                   & 0.028                                                        \\
                                                            & \dataaugwithhuman    & 65.9                                                    & 0.059                                                         & 57.5                                                   & 0.103                                                        \\ \hline
\end{tabular}
\end{table*}

==> tables/fake_example_table.tex <==
\begin{table*}[]
\tiny
\begin{tabular}{@{}p{0.23\linewidth} p{0.23\linewidth} p{0.23\linewidth} p{0.23\linewidth}@{}}
\toprule
\multicolumn{1}{c}{\textbf{Human rationale}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               & \multicolumn{1}{c}{\textbf{Attack tokens}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            & \multicolumn{1}{c}{\textbf{Human-supervised model}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                & \multicolumn{1}{c}{\textbf{Attack-supervised model}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \midrule
\multicolumn{4}{c}{\textbf{(A) Scenario 1}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \midrule
\definecolor{highlight}{RGB}{250, 215, 160 }\sethlcolor{highlight}\hl{{[}CLS{]}}\xspace\xspace\xspace...\xspace\xspace \hl{in}\hl{ }\hl{may}\hl{ }\hl{1904}\hl{ }\hl{,}\hl{ }\hl{the}\hl{ }\hl{couple}\hl{ }\hl{'}\hl{ }\hl{s}\hl{ }\hl{first}\hl{ }\hl{son}\hl{ }\hl{,}\hl{ }\hl{hans}\hl{ }\hl{albert}\hl{ }\hl{einstein}\hl{ }\hl{,}\hl{ }\hl{was}\hl{ }\hl{born}\hl{ }\hl{in}\hl{ }\hl{bern}\hl{ }\hl{,}\hl{ }\hl{switzerland}\hl{ }\hl{.}\hl{ }\hl{their}\hl{ }\hl{second}\hl{ }\hl{son}\hl{ }\hl{,}\hl{ }\hl{eduard}\hl{ }\hl{,}\hl{ }\hl{was}\hl{ }\hl{born}\hl{ }\hl{in}\hl{ }\hl{zurich}\hl{ }\hl{in}\hl{ }\hl{july}\hl{ }\hl{1910}\hl{ }\hl{.}\hl{ }\hl{in}\hl{ }\hl{1914}\hl{ }\hl{,}\hl{ }\hl{the}\hl{ }\hl{couple}\hl{ }\hl{separated}\hl{ }\hl{;}\hl{ }\hl{einstein}\hl{ }\hl{moved}\hl{ }\hl{to}\hl{ }\hl{berlin}\hl{ }\hl{and}\hl{ }\hl{his}\hl{ }\hl{wife}\hl{ }\hl{remained}\hl{ }\hl{in}\hl{ }\hl{zurich}\hl{ }\hl{with}\hl{ }\hl{their}\hl{ }\hl{sons}\hl{ }\hl{.} they divorced on 14 february 1919 , having lived apart for five years .\xspace\xspace\xspace...\xspace\xspace a - tete did n ' t stay in basel after charles and houben separated .\xspace\xspace\xspace...\xspace\xspace \hl{{[}SEP{]}}\hl{ }\hl{who}\hl{ }\hl{did}\hl{ }\hl{n}\hl{ }\hl{'}\hl{ }\hl{t}\hl{ }\hl{stay}\hl{ }\hl{in}\hl{ }\hl{zurich}\hl{ }\hl{after}\hl{ }\hl{albert}\hl{ }\hl{and}\hl{ }\hl{mari}\hl{c}\hl{ }\hl{separated}\hl{ }\hl{?}\hl{ }\hl{|}\hl{ }\hl{|}\hl{ }\hl{te}\hl{te}\hl{ }\hl{{[}SEP{]}}                                           & \definecolor{highlight}{RGB}{230, 176, 170}\sethlcolor{highlight}{[}CLS{]}\xspace\xspace\xspace...\xspace\xspace in may 1904 , the couple ' s first son , hans albert einstein , was born in bern , switzerland . their second son , eduard , was born in zurich in july 1910 . in 1914 , the couple separated ; einstein moved to berlin and his wife remained in zurich with their sons . they divorced on 14 february 1919 , having lived apart for five years .\xspace\xspace\xspace...\xspace\xspace \hl{a}\hl{ }\hl{-}\hl{ }\hl{te}\hl{te}\hl{ }\hl{did}\hl{ }\hl{n}\hl{ }\hl{'}\hl{ }\hl{t}\hl{ }\hl{stay}\hl{ }\hl{in}\hl{ }\hl{basel}\hl{ }\hl{after}\hl{ }\hl{charles}\hl{ }\hl{and}\hl{ }\hl{ho}\hl{ub}\hl{en}\hl{ }\hl{separated}\hl{ }\hl{.}\xspace\xspace\xspace...\xspace\xspace {[}SEP{]} who did n ' t stay in zurich after albert and maric separated ? | | tete {[}SEP{]} & \definecolor{highlight}{RGB}{154,205,50}\sethlcolor{highlight}\hl{{[}CLS{]}}\xspace\xspace\xspace...\xspace\xspace in may 1904 , the couple ' s first son , hans albert einstein , was born in bern , switzerland . their second son , eduard , was born in zurich in july 1910 \hl{.}\hl{ }\hl{in}\hl{ }\hl{1914}\hl{ }\hl{,}\hl{ }\hl{the}\hl{ }\hl{couple}\hl{ }\hl{separated}\hl{ }\hl{;}\hl{ }\hl{einstein}\hl{ }\hl{moved}\hl{ }\hl{to}\hl{ }\hl{berlin}\hl{ }\hl{and}\hl{ }\hl{his}\hl{ }\hl{wife}\hl{ }\hl{remained}\hl{ }\hl{in}\hl{ }\hl{zurich}\hl{ }\hl{with}\hl{ }\hl{their}\hl{ }\hl{sons}\hl{ }\hl{.}\hl{ }\hl{they}\hl{ }\hl{divorced}\hl{ }\hl{on}\hl{ }\hl{14}\hl{ }\hl{february}\hl{ }\hl{1919}\hl{ }\hl{,}\hl{ }\hl{having}\hl{ }\hl{lived}\hl{ }\hl{apart}\hl{ }\hl{for}\hl{ }\hl{five}\hl{ }\hl{years}\hl{ }\hl{.}\xspace\xspace\xspace...\xspace\xspace a - tete did n ' t stay in basel after charles and houben separated .\xspace\xspace\xspace...\xspace\xspace \hl{{[}SEP{]}}\hl{ }\hl{who}\hl{ }\hl{did}\hl{ }\hl{n}\hl{ }\hl{'}\hl{ }\hl{t}\hl{ }\hl{stay}\hl{ }\hl{in}\hl{ }\hl{zurich}\hl{ }\hl{after}\hl{ }\hl{albert}\hl{ }\hl{and}\hl{ }\hl{mari}\hl{c}\hl{ }\hl{separated}\hl{ }\hl{?}\hl{ }\hl{|}\hl{ }\hl{|}\hl{ }\hl{te}\hl{te}\hl{ }\hl{{[}SEP{]}}                                                                                                                                                                                                                                                                                                                   & \definecolor{highlight}{RGB}{169, 204, 227}\sethlcolor{highlight}\hl{{[}CLS{]}}\xspace\xspace\xspace...\xspace\xspace\hl{ }\hl{in}\hl{ }\hl{may}\hl{ }\hl{1904}\hl{ }\hl{,}\hl{ }\hl{the}\hl{ }\hl{couple}\hl{ }\hl{'}\hl{ }\hl{s}\hl{ }\hl{first}\hl{ }\hl{son}\hl{ }\hl{,}\hl{ }\hl{hans}\hl{ }\hl{albert}\hl{ }\hl{einstein}\hl{ }\hl{,}\hl{ }\hl{was}\hl{ }\hl{born}\hl{ }\hl{in}\hl{ }\hl{bern}\hl{ }\hl{,}\hl{ }\hl{switzerland}\hl{ }\hl{.}\hl{ }\hl{their}\hl{ }\hl{second}\hl{ }\hl{son}\hl{ }\hl{,}\hl{ }\hl{eduard}\hl{ }\hl{,}\hl{ }\hl{was}\hl{ }\hl{born}\hl{ }\hl{in}\hl{ }\hl{zurich}\hl{ }\hl{in}\hl{ }\hl{july}\hl{ }\hl{1910}\hl{ }\hl{.}\hl{ }\hl{in}\hl{ }\hl{1914}\hl{ }\hl{,}\hl{ }\hl{the}\hl{ }\hl{couple}\hl{ }\hl{separated}\hl{ }\hl{;}\hl{ }\hl{einstein}\hl{ }\hl{moved}\hl{ }\hl{to}\hl{ }\hl{berlin}\hl{ }\hl{and}\hl{ }\hl{his}\hl{ }\hl{wife}\hl{ }\hl{remained}\hl{ }\hl{in}\hl{ }\hl{zurich}\hl{ }\hl{with}\hl{ }\hl{their}\hl{ }\hl{sons}\hl{ }\hl{.}\hl{ }\hl{they}\hl{ }\hl{divorced}\hl{ }\hl{on}\hl{ }\hl{14}\hl{ }\hl{february}\hl{ }\hl{1919}\hl{ }\hl{,}\hl{ }\hl{having}\hl{ }\hl{lived}\hl{ }\hl{apart}\hl{ }\hl{for}\hl{ }\hl{five}\hl{ }\hl{years}\hl{ }\hl{.}\xspace\xspace\xspace...\xspace\xspace a - tete did n ' t stay in basel after charles and houben separated .\xspace\xspace\xspace...\xspace\xspace\hl{ }\hl{{[}SEP{]}}\hl{ }\hl{who}\hl{ }\hl{did}\hl{ }\hl{n}\hl{ }\hl{'}\hl{ }\hl{t}\hl{ }\hl{stay}\hl{ }\hl{in}\hl{ }\hl{zurich}\hl{ }\hl{after}\hl{ }\hl{albert}\hl{ }\hl{and}\hl{ }\hl{mari}\hl{c}\hl{ }\hl{separated}\hl{ }\hl{?}\hl{ }\hl{|}\hl{ }\hl{|}\hl{ }\hl{te}\hl{te}\hl{ }\hl{{[}SEP{]}} \\
\textbf{Label: False}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \textbf{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             & \textbf{Outcome: False}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            & \textbf{Outcome: False}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \midrule
\multicolumn{4}{c}{\textbf{(B) Scenario 2}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \midrule
\definecolor{highlight}{RGB}{250, 215, 160 }\sethlcolor{highlight}\hl{{[}CLS{]}}\xspace\xspace\xspace...\xspace\xspace \hl{on}\hl{ }\hl{the}\hl{ }\hl{day}\hl{ }\hl{of}\hl{ }\hl{the}\hl{ }\hl{party}\hl{ }\hl{,}\hl{ }\hl{all}\hl{ }\hl{five}\hl{ }\hl{friends}\hl{ }\hl{showed}\hl{ }\hl{up}\hl{ }\hl{.}\hl{ }\hl{each}\hl{ }\hl{friend}\hl{ }\hl{had}\hl{ }\hl{a}\hl{ }\hl{present}\hl{ }\hl{for}\hl{ }\hl{susan}\hl{ }\hl{.} 6 thank - you cards did helen send . \hl{susan}\hl{ }\hl{was}\hl{ }\hl{happy}\hl{ }\hl{and}\hl{ }\hl{sent}\hl{ }\hl{each}\hl{ }\hl{friend}\hl{ }\hl{a}\hl{ }\hl{thank}\hl{ }\hl{you}\hl{ }\hl{card}\hl{ }\hl{the}\hl{ }\hl{next}\hl{ }\hl{week}\hl{ }\hl{.}\hl{ }\hl{{[}SEP{]}}\hl{ }\hl{how}\hl{ }\hl{many}\hl{ }\hl{thank}\hl{ }\hl{-}\hl{ }\hl{you}\hl{ }\hl{cards}\hl{ }\hl{did}\hl{ }\hl{susan}\hl{ }\hl{send}\hl{ }\hl{?}\hl{ }\hl{|}\hl{ }\hl{|}\hl{ }\hl{5}\hl{ }\hl{{[}SEP{]}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             & \definecolor{highlight}{RGB}{230, 176, 170}\sethlcolor{highlight}{[}CLS{]}\xspace\xspace\xspace...\xspace\xspace on the day of the party , all five friends showed up . each friend had a present for susan . \hl{6}\hl{ }\hl{thank}\hl{ }\hl{-}\hl{ }\hl{you}\hl{ }\hl{cards}\hl{ }\hl{did}\hl{ }\hl{helen}\hl{ }\hl{send}\hl{ }\hl{.} susan was happy and sent each friend a thank you card the next week . {[}SEP{]} how many thank - you cards did susan send ? | | 5 {[}SEP{]}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 & \definecolor{highlight}{RGB}{154,205,50}\sethlcolor{highlight}\hl{{[}CLS{]}}\xspace\xspace\xspace...\xspace\xspace on the day of the party , all five friends showed up . each friend had a present for susan . 6 thank - you cards did helen send . \hl{susan}\hl{ }\hl{was}\hl{ }\hl{happy}\hl{ }\hl{and}\hl{ }\hl{sent}\hl{ }\hl{each}\hl{ }\hl{friend}\hl{ }\hl{a}\hl{ }\hl{thank}\hl{ }\hl{you}\hl{ }\hl{card}\hl{ }\hl{the}\hl{ }\hl{next}\hl{ }\hl{week}\hl{ }\hl{.}\hl{ }\hl{{[}SEP{]}}\hl{ }\hl{how}\hl{ }\hl{many}\hl{ }\hl{thank}\hl{ }\hl{-}\hl{ }\hl{you}\hl{ }\hl{cards}\hl{ }\hl{did}\hl{ }\hl{susan}\hl{ }\hl{send}\hl{ }\hl{?}\hl{ }\hl{|}\hl{ }\hl{|}\hl{ }\hl{5}\hl{ }\hl{{[}SEP{]}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               & \definecolor{highlight}{RGB}{169, 204, 227}\sethlcolor{highlight}\hl{{[}CLS{]}}\xspace\xspace\xspace...\xspace\xspace\hl{ }\hl{on}\hl{ }\hl{the}\hl{ }\hl{day}\hl{ }\hl{of}\hl{ }\hl{the}\hl{ }\hl{party}\hl{ }\hl{,}\hl{ }\hl{all}\hl{ }\hl{five}\hl{ }\hl{friends}\hl{ }\hl{showed}\hl{ }\hl{up}\hl{ }\hl{.}\hl{ }\hl{each}\hl{ }\hl{friend}\hl{ }\hl{had}\hl{ }\hl{a}\hl{ }\hl{present}\hl{ }\hl{for}\hl{ }\hl{susan}\hl{ }\hl{.} 6 thank - you cards did helen send . \hl{susan}\hl{ }\hl{was}\hl{ }\hl{happy}\hl{ }\hl{and}\hl{ }\hl{sent}\hl{ }\hl{each}\hl{ }\hl{friend}\hl{ }\hl{a}\hl{ }\hl{thank}\hl{ }\hl{you}\hl{ }\hl{card}\hl{ }\hl{the}\hl{ }\hl{next}\hl{ }\hl{week}\hl{ }\hl{.}\hl{ }\hl{{[}SEP{]}}\hl{ }\hl{how}\hl{ }\hl{many}\hl{ }\hl{thank}\hl{ }\hl{-}\hl{ }\hl{you}\hl{ }\hl{cards}\hl{ }\hl{did}\hl{ }\hl{susan}\hl{ }\hl{send}\hl{ }\hl{?}\hl{ }\hl{|}\hl{ }\hl{|}\hl{ }\hl{5}\hl{ }\hl{{[}SEP{]}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\
\textbf{Label: True}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & \textbf{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             & \textbf{Outcome: False}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            & \textbf{Outcome: True}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \midrule
\multicolumn{4}{c}{\textbf{(C) Scenario 3}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \midrule
\definecolor{highlight}{RGB}{250, 215, 160 }\sethlcolor{highlight}\hl{{[}CLS{]}}\xspace\xspace\xspace...\xspace\xspace \hl{roman}\hl{ }\hl{legions}\hl{ }\hl{encountered}\hl{ }\hl{the}\hl{ }\hl{stronghold}\hl{s}\hl{ }\hl{of}\hl{ }\hl{the}\hl{ }\hl{castle}\hl{ }\hl{rock}\hl{ }\hl{and}\hl{ }\hl{arthur}\hl{ }\hl{'}\hl{ }\hl{s}\hl{ }\hl{seat}\hl{ }\hl{,}\hl{ }\hl{held}\hl{ }\hl{by}\hl{ }\hl{a}\hl{ }\hl{tribe}\hl{ }\hl{of}\hl{ }\hl{ancient}\hl{ }\hl{brit}\hl{ons}\hl{ }\hl{known}\hl{ }\hl{as}\hl{ }\hl{the}\hl{ }\hl{vo}\hl{tad}\hl{ini}\hl{ }\hl{.} the mercians were probably the ancestors of the manaw . \hl{little}\hl{ }\hl{is}\hl{ }\hl{recorded}\hl{ }\hl{about}\hl{ }\hl{this}\hl{ }\hl{group}\hl{ }\hl{,}\hl{ }\hl{but}\hl{ }\hl{they}\hl{ }\hl{were}\hl{ }\hl{probably}\hl{ }\hl{the}\hl{ }\hl{ancestors}\hl{ }\hl{of}\hl{ }\hl{the}\hl{ }\hl{god}\hl{od}\hl{din}\hl{ }\hl{,}\hl{ }\hl{whose}\hl{ }\hl{feat}\hl{s}\hl{ }\hl{are}\hl{ }\hl{told}\hl{ }\hl{in}\hl{ }\hl{a}\hl{ }\hl{seventh}\hl{ }\hl{-}\hl{ }\hl{century}\hl{ }\hl{old}\hl{ }\hl{welsh}\hl{ }\hl{manuscript}\hl{ }\hl{.}\xspace\xspace\xspace...\xspace\xspace the god\xspace\xspace\xspace...\xspace\xspacedin\xspace\xspace\xspace...\xspace\xspace \hl{{[}SEP{]}}\hl{ }\hl{who}\hl{ }\hl{were}\hl{ }\hl{probably}\hl{ }\hl{the}\hl{ }\hl{ancestors}\hl{ }\hl{of}\hl{ }\hl{the}\hl{ }\hl{god}\hl{od}\hl{din}\hl{ }\hl{?}\hl{ }\hl{|}\hl{ }\hl{|}\hl{ }\hl{the}\hl{ }\hl{pic}\hl{ts}\hl{ }\hl{{[}SEP{]}} & \definecolor{highlight}{RGB}{230, 176, 170}\sethlcolor{highlight}{[}CLS{]}\xspace\xspace\xspace...\xspace\xspace roman legions encountered the strongholds of the castle rock and arthur ' s seat , held by a tribe of ancient britons known as the votadini . \hl{the}\hl{ }\hl{mer}\hl{cian}\hl{s}\hl{ }\hl{were}\hl{ }\hl{probably}\hl{ }\hl{the}\hl{ }\hl{ancestors}\hl{ }\hl{of}\hl{ }\hl{the}\hl{ }\hl{mana}\hl{w}\hl{ }\hl{.} little is recorded about this group , but they were probably the ancestors of the gododdin , whose feats are told in a seventh - century old welsh manuscript .\xspace\xspace\xspace...\xspace\xspace the god\xspace\xspace\xspace...\xspace\xspacedin\xspace\xspace\xspace...\xspace\xspace {[}SEP{]} who were probably the ancestors of the gododdin ? | | the picts {[}SEP{]}                                                                                                                                                                                                         & \definecolor{highlight}{RGB}{154,205,50}\sethlcolor{highlight}\hl{{[}CLS{]}}\xspace\xspace\xspace...\xspace\xspace roman legions encountered the strongholds of the castle rock and arthur ' s seat , held by a tribe of ancient britons known as the votadini . \hl{the}\hl{ }\hl{mer}\hl{cian}\hl{s}\hl{ }\hl{were}\hl{ }\hl{probably}\hl{ }\hl{the}\hl{ }\hl{ancestors}\hl{ }\hl{of}\hl{ }\hl{the}\hl{ }\hl{mana}\hl{w}\hl{ }\hl{.}\hl{ }\hl{little}\hl{ }\hl{is}\hl{ }\hl{recorded}\hl{ }\hl{about}\hl{ }\hl{this}\hl{ }\hl{group}\hl{ }\hl{,}\hl{ }\hl{but}\hl{ }\hl{they}\hl{ }\hl{were}\hl{ }\hl{probably}\hl{ }\hl{the}\hl{ }\hl{ancestors}\hl{ }\hl{of}\hl{ }\hl{the}\hl{ }\hl{god}\hl{od}\hl{din}\hl{ }\hl{,}\hl{ }\hl{whose}\hl{ }\hl{feat}\hl{s}\hl{ }\hl{are}\hl{ }\hl{told}\hl{ }\hl{in}\hl{ }\hl{a}\hl{ }\hl{seventh}\hl{ }\hl{-}\hl{ }\hl{century}\hl{ }\hl{old}\hl{ }\hl{welsh}\hl{ }\hl{manuscript}\hl{ }\hl{.}\xspace\xspace\xspace...\xspace\xspace \hl{the}\hl{ }\hl{god}\xspace\xspace\xspace...\xspace\xspace\hl{din}\xspace\xspace\xspace...\xspace\xspace \hl{{[}SEP{]}}\hl{ }\hl{who}\hl{ }\hl{were}\hl{ }\hl{probably}\hl{ }\hl{the}\hl{ }\hl{ancestors}\hl{ }\hl{of}\hl{ }\hl{the}\hl{ }\hl{god}\hl{od}\hl{din}\hl{ }\hl{?}\hl{ }\hl{|}\hl{ }\hl{|}\hl{ }\hl{the}\hl{ }\hl{pic}\hl{ts}\hl{ }\hl{{[}SEP{]}} & \definecolor{highlight}{RGB}{169, 204, 227}\sethlcolor{highlight}\hl{{[}CLS{]}}\xspace\xspace\xspace...\xspace\xspace\hl{ }\hl{roman}\hl{ }\hl{legions}\hl{ }\hl{encountered}\hl{ }\hl{the}\hl{ }\hl{stronghold}\hl{s}\hl{ }\hl{of}\hl{ }\hl{the}\hl{ }\hl{castle}\hl{ }\hl{rock}\hl{ }\hl{and}\hl{ }\hl{arthur}\hl{ }\hl{'}\hl{ }\hl{s}\hl{ }\hl{seat}\hl{ }\hl{,}\hl{ }\hl{held}\hl{ }\hl{by}\hl{ }\hl{a}\hl{ }\hl{tribe}\hl{ }\hl{of}\hl{ }\hl{ancient}\hl{ }\hl{brit}\hl{ons}\hl{ }\hl{known}\hl{ }\hl{as}\hl{ }\hl{the}\hl{ }\hl{vo}\hl{tad}\hl{ini}\hl{ }\hl{.} the mercians were probably the ancestors of the manaw . \hl{little}\hl{ }\hl{is}\hl{ }\hl{recorded}\hl{ }\hl{about}\hl{ }\hl{this}\hl{ }\hl{group}\hl{ }\hl{,}\hl{ }\hl{but}\hl{ }\hl{they}\hl{ }\hl{were}\hl{ }\hl{probably}\hl{ }\hl{the}\hl{ }\hl{ancestors}\hl{ }\hl{of}\hl{ }\hl{the}\hl{ }\hl{god}\hl{od}\hl{din}\hl{ }\hl{,}\hl{ }\hl{whose}\hl{ }\hl{feat}\hl{s}\hl{ }\hl{are}\hl{ }\hl{told}\hl{ }\hl{in}\hl{ }\hl{a}\hl{ }\hl{seventh}\hl{ }\hl{-}\hl{ }\hl{century}\hl{ }\hl{old}\hl{ }\hl{welsh}\hl{ }\hl{manuscript}\hl{ }\hl{.}\xspace\xspace\xspace...\xspace\xspace\hl{ }\hl{the}\hl{ }\hl{god}\xspace\xspace\xspace...\xspace\xspace\hl{din}\xspace\xspace\xspace...\xspace\xspace\hl{ }\hl{{[}SEP{]}}\hl{ }\hl{who}\hl{ }\hl{were}\hl{ }\hl{probably}\hl{ }\hl{the}\hl{ }\hl{ancestors}\hl{ }\hl{of}\hl{ }\hl{the}\hl{ }\hl{god}\hl{od}\hl{din}\hl{ }\hl{?}\hl{ }\hl{|}\hl{ }\hl{|}\hl{ }\hl{the}\hl{ }\hl{pic}\hl{ts}\hl{ }\hl{{[}SEP{]}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\
\textbf{Label: False  }                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & \textbf{Outcome: False}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            & \textbf{Outcome: True}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \bottomrule
\end{tabular}


\caption{Example outputs from ...}
\label{tab:fake_example_table}
\end{table*}

==> tables/multirc-random-100.tex <==
\begin{table*}[]
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
model\_alias & test & adversarial-squad-start & adversarial-squad-random & adversarial-squad-end \\ \midrule
BC              & 0.673 & 0.615 & 0.616 & 0.626 \\
BR-sup          & 0.697 & 0.677 & 0.684 & 0.685 \\
BR-sup-sigmoid  & 0.705 & 0.692 & 0.694 & 0.695 \\
BSR-sup         & 0.703 & 0.690 & 0.691 & 0.686 \\
BSR-sup-sigmoid & 0.682 & 0.644 & 0.655 & 0.656 \\
RC              & 0.844 & 0.829 & 0.829 & 0.832 \\
RR-sup          & 0.838 & 0.841 & 0.840 & 0.840 \\
RR-sup-sigmoid  & 0.850 & 0.831 & 0.825 & 0.842 \\
RSR-sup         & 0.828 & 0.820 & 0.811 & 0.821 \\
RSR-sup-sigmoid & 0.839 & 0.838 & 0.835 & 0.834 \\ \bottomrule
\end{tabular}
\caption{Finetuning on MultiRC dataset augmented by adversarial-squad-random attack}
\label{tab:multirc-random}
\end{table*}

==> tables/multirc-random-all-rationale.tex <==

\begin{table*}[]
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
model\_alias & test & adversarial-squad-start & adversarial-squad-random & adversarial-squad-end \\ \midrule
BC              & 0.673 & 0.615 & 0.616 & 0.626 \\
BR-sup          & 0.678 & 0.664 & 0.670 & 0.661 \\
BR-sup-sigmoid  & 0.696 & 0.658 & 0.662 & 0.656 \\
BSR-sup         & 0.672 & 0.650 & 0.657 & 0.649 \\
BSR-sup-sigmoid & 0.689 & 0.643 & 0.641 & 0.648 \\
RC              & 0.844 & 0.829 & 0.829 & 0.832 \\
RR-sup          & 0.824 & 0.844 & 0.840 & 0.840 \\
RR-sup-sigmoid  & 0.852 & 0.857 & 0.851 & 0.850 \\
RSR-sup         & 0.832 & 0.849 & 0.849 & 0.848 \\
RSR-sup-sigmoid & 0.824 & 0.854 & 0.848 & 0.847 \\ \bottomrule
\end{tabular}
\caption{Finetuning on MultiRC dataset augmented by adversarial-squad-random attack where all input tokens are labeled as true rationale}
\label{tab:multirc-random-all-rationale}
\end{table*}

==> tables/multirc.tex <==
% notebook/get_all_numbers_multirc_best.ipynb
\begin{table*}[]
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
model\    & test  & adversarial-squad-start & adversarial-squad-random & adversarial-squad-end \\ \midrule
BC              & 0.686 & 0.619                   & 0.626                    & 0.636                 \\
BR-sup          & 0.692 & 0.631                   & 0.637                    & 0.669                 \\
BR-sup-sigmoid  & 0.700 & 0.632                   & 0.644                    & 0.668                 \\
BSR-sup         & 0.698 & 0.611                   & 0.629                    & 0.652                 \\
BSR-sup-sigmoid & 0.697 & 0.630                   & 0.642                    & 0.666                 \\
RC              & 0.826 & 0.760                   & 0.765                    & 0.779                 \\
RR-sup          & 0.819 & 0.724                   & 0.727                    & 0.756                 \\
RR-sup-sigmoid  & 0.840 & 0.753                   & 0.749                    & 0.776                 \\
RSR-sup         & 0.816 & 0.720                   & 0.714                    & 0.748                 \\
RSR-sup-sigmoid & 0.830 & 0.741                   & 0.736                    & 0.760                 \\ \bottomrule
\end{tabular}
\caption{MultiRC numbers for all models. Hyperparameters are chosen from a grid search, and model with the best dev accuracy among three random seeds is reported.}
\label{tab:multirc}
\end{table*}

==> tables/recall.tex <==
\begin{table*}[]
\begin{tabular}{llllll}
\hline
Model                                                       & Augmentation                        & \begin{tabular}[c]{@{}l@{}}Attack\\ Recall\end{tabular} & \begin{tabular}[c]{@{}l@{}}Attack\\ Recall Corr.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Human\\ Recall\end{tabular} & \begin{tabular}[c]{@{}l@{}}Human\\ Recall Corr.\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Bert Rationale\end{tabular}    & \humantokens         & 11.2                                                    & 0.032                                                         & 35.8                                                   & 0.104                                                        \\
                                                            & \dataaugwithnatokens & 97.4                                                    & -0.055                                                        & 98.6                                                   & -0.011                                                       \\
                                                            & \dataaugwithhuman    & 89.3                                                    & -0.053                                                        & 57.6                                                   & 0.092                                                        \\ \hline
\begin{tabular}[c]{@{}l@{}}RoBERTa Rationale\end{tabular} & \humantokens         & 5.6                                                     & 0.043                                                         & 46.6                                                   & 0.148                                                        \\
                                                            & \dataaugwithnatokens & 92.1                                                    & -0.029                                                        & 97.3                                                   & 0.028                                                        \\
                                                            & \dataaugwithhuman    & 65.9                                                    & 0.059                                                         & 57.5                                                   & 0.103                                                        \\ \hline
\end{tabular}
\end{table*}
